Online Stochastic Matching: New Algorithms and Bounds

Online matching has received significant attention over the last 15 years due to its close connection to Internet advertising. As the seminal work of Karp, Vazirani, and Vazirani has an optimal (1 - 1/e) competitive ratio in the standard adversarial online model, much effort has gone into developing useful online models that incorporate some stochasticity in the arrival process. One such popular model is the "known I.I.D. model" where different customer-types arrive online from a known distribution. We develop algorithms with improved competitive ratios for some basic variants of this model with integral arrival rates, including (a) the case of general weighted edges, where we improve the best-known ratio of 0.667 due to Haeupler, Mirrokni and Zadimoghaddam to 0.705; and (b) the vertex-weighted case, where we improve the 0.7250 ratio of Jaillet and Lu to 0.7299. We also consider an extension of stochastic rewards, a variant where each edge has an independent probability of being present. For the setting of stochastic rewards with non-integral arrival rates, we present a simple optimal non-adaptive algorithm with a ratio of 1 - 1/e. For the special case where each edge is unweighted and has a uniform constant probability of being present, we improve upon 1 - 1/e by proposing a strengthened LP benchmark.

==> 01-abstract.tex <==
Online matching has received significant attention in recent years due to its close connection to Internet advertising. As the seminal work of Karp, Vazirani, and Vazirani has an optimal $(1 - 1/\euler)$ competitive ratio in the standard adversarial online model, much effort has gone into developing useful online models that incorporate some stochasticity in the arrival process. One such popular model is the ``known I.I.D. model'' where different customer-types arrive online from a known distribution. We develop algorithms with improved competitive ratios for some basic variants of this model with integral arrival rates, including: (a) the case of general weighted edges, where we improve the best-known ratio of $0.667$ due to Haeupler, Mirrokni and Zadimoghaddam (\emph{WINE}, 2011) to $0.705$; and (b) the vertex-weighted case, where we improve the $0.7250$ ratio of Jaillet and Lu (\emph{Mathematics of Operations Research}, 2013) to $0.7299$. 
We also consider an extension of stochastic rewards, a variant where each edge has an
 independent probability of being present. For the setting of stochastic rewards with non-integral arrival rates, we present a simple \emph{optimal} non-adaptive algorithm with a ratio of $1-1/\euler$. For the special case where each edge is unweighted and has a uniform constant probability of being present, we improve upon $1-1/\euler$ by proposing a strengthened LP benchmark.

%We also consider two extensions, one is ``known I.I.D.'' with non-integral arrival rate and stochastic rewards; the other is ``known I.I.D.''  $b$-matching with non-integral arrival rate and stochastic rewards. We present a simple non-adaptive algorithm which works well simultaneously on the two extensions.

One of the key ingredients of our improvement is the following (offline) approach to bipartite-matching polytopes with additional constraints. We first add several valid constraints in order to get a good fractional solution $\ff$; however, these give us less control over the structure of $\ff$. We next \emph{remove} all these additional constraints and randomly move from $\textbf{f}$ to a feasible point on the matching polytope with all coordinates being from the set $\{0, 1/k, 2/k, \ldots, 1\}$ for a chosen integer $k$. The structure of this solution is inspired by Jaillet and Lu (\emph{Mathematics of Operations Research}, 2013) and is a tractable structure for algorithm design and analysis. The appropriate random move preserves many of the removed constraints (approximately with high probability and exactly in expectation). This underlies some of our improvements and could be of independent interest.


==> 6-bmat.tex <==




\section{Extension to $b$-matching  with stochastic rewards}
\label{sec:b-matching}
In this section, we further generalize the model in Section~\ref{sec:nonint} to the case where each $u$ in the offline set $U$ has a uniform integral capacity $b$ (i.e., each vertex $u$ can be matched at most $b$ times). Otherwise, we retain the same setting as Section~\ref{sec:nonint}; we allow non-integral arrival rates and stochastic rewards. We will generalize the simple algorithm used in the previous setting (i.e., Section~\ref{sec:nonint}) to this new setting. \\

Consider the following updated LP:
% \ref{lp2:stoch-match} 
\begin{eqnarray}
	\label{lp:stoch-b-match}
	\max && \sum_{e \in E} w_{e} f_e p_e: \\
	\mbox{s.t.} &&
	\sum_{e \in \partial(u)} f_e p_{e} \leq b, \forall u \in U \\
	&& \sum_{e \in \partial(v)} f_e \leq r_{v}, \forall v \in V \\
\end{eqnarray}


We modify Algorithm \ref{alg:non-integral} for the $b$-matching problem as follows.
\begin{algorithm}[!h]
	
	\caption{$\mathsf{SM_b}$}\label{alg:b-non-integral}
	\DontPrintSemicolon
	Construct and solve LP~\eqref{lp:stoch-b-match}. WLOG assume 
	$\{f_{e}| e \in E\}$ is an optimal solution. \;
	
	When a vertex $v$ arrives, assign $v$ to each of its neighbor $u$ with a probability $\frac{f_{(u,v)}}{r_v}$. \; \label{alg: b-step2}
\end{algorithm}

Let us now prove Theorem \ref{thm:b-non-integral}. 
\begin{proof}
	The proof is similar to that of Theorem \ref{thm:non-integral}. Let 
	$A_t$ be the number of times $u$ has been matched at the beginning of round $t$.
	%Suppose we call $u$ is safe at the beginning of $t$ iff $A_t \le b-1$. 
	Let $B(u,t)$ be the event that $u$ is safe at  the beginning of round $t$, which is defined as $A_t \le b-1$.  For any given edge $e$, let $X_e$ be the number of times that $e$ gets matched over the $n$ rounds. 
	Thus we have
	$$\E[X_e] = \sum_{t=1}^n
	\Pr[B(u,t)] \frac{r_v}{n} \frac{f_e}{r_v} p_e=
	\frac{f_ep_e}{n}\sum_{t=1}^n \Pr[A_t \le b-1]$$
	
	Now we upper bound the value of $\Pr[A_t \ge b]$. 
	For each $1 \le i \le t$, let $Z_i$ be the indicator random variable for $u$ to be matched during round $i$. Thus $A_{t+1}=\sum_{i=1}^{t} Z_i$. Notice that for each $i$, we have 
	\[
	\E[Z_i]\le \sum_{v \sim u}\frac{r_v}{n} \frac{f_{(u,v)}}{r_v} p_{(u,v)}  \le \frac{b}{n}
	\]
	It follows that for any $t \le n(1-\tau)$ with $0<\tau<1$, we have $\E[A_{t+1}] \le (1-\tau)b$. By applying Chernoff-Hoeffding bounds, we get
	$\Pr[A_{t+1} \ge b] \le e^{-b \tau^2/3}$. Therefore
	\begin{align*}
		\E[X_e] 
		&= \frac{f_ep_e}{n}\sum_{t=1}^n \Pr[A_t \le b-1] \\
		&\geq \frac{f_ep_e}{n}\sum_{t=1}^{n(1-\tau)} (1-e^{-b \tau^2/3}) 
		= f_e p_e (1-\tau)(1-e^{-b \tau^2/3})
	\end{align*}
	For any given $\epsilon>0$, choose $\tau=b^{-1/2+\epsilon}$ to get a competitive ratio of $1-b^{-1/2+\epsilon}-O(e^{-b^{2\epsilon}/3})$.
\end{proof}



